DDPNOpt: Differential Dynamic Programming Neural Optimizer

Interpretation of Deep Neural Networks (DNNs) training as an optimal control problem with nonlinear dynamical systems has received considerable attention recently, yet the algorithmic development remains relatively limited. In this work, we make an attempt along this line by reformulating the training procedure from the trajectory optimization perspective. We first show that most widely-used algorithms for training DNNs can be linked to the Differential Dynamic Programming (DDP), a celebrated second-order method rooted in the Approximate Dynamic Programming. In this vein, we propose a new class of optimizer, DDP Neural Optimizer (DDPNOpt), for training feedforward and convolution networks. DDPNOpt features layer-wise feedback policies which improve convergence and reduce sensitivity to hyper-parameter over existing methods. It outperforms other optimal-control inspired training methods in both convergence and complexity, and is competitive against state-of-the-art first and second order methods. We also observe DDPNOpt has surprising benefit in preventing gradient vanishing. Our work opens up new avenues for principled algorithmic design built upon the optimal control theory.

==> rebuttal.tex <==

**Author response to all reviewers**

We thank the reviewers for their valuable comments. We are excited that the reviewers identified the novelty of the connection (R1,R2,R3,R4), comprehensive experiments (R3,R4), and well-written presentation (R1,R2,R3,R4) of our work. We believe DDPNOpt takes a significant step toward new algorithmic design inspired from optimal control.

We address raised concerns and revise the submission with the modifications marked as blue. Below we summarize the changes in the revision.

1. Following R4's suggestion on increasing the reading experience for broader audience,
we introduce DDPNOpt right after we present the connection between vanilla DDP and existing methods (Proposition 2),
so that the derivation of DDPNOpt is close to DDP, making it easier to compare between three frameworks.
Discussion on 'Role of the feedback $K_t$ and $\delta x_t$' (i.e. the latter part of Sec 3 in the original submission) now appears after the derivation of DDPNOpt.

2. The pseudo-code of DDPNOpt is now attached in page 6 (Alg. 3), with the computation at each stage linked to the corresponding equation. We also include additional discussion on the Vxx regularization.

3. Clarifications on experiment setups and minor typos in figures are included in Sec 5. Additional experiments and discussions raised by each reviewer are left in Appendix A.7.

4. Minor clarifications on notation and expanding point are added in Sec 2.


====================== R1 =======================

**  **

** Vanishing gradient experiment **


====================== R2 =======================

We greatly thank R2 for the very helpful and detailed suggestions.


Fig 4 is corrected where we identified misleading values for 2 learning rates. We attach numerical values in Appendix A.7.3.

[calrification of runtime experiment ]


[calrification of memory experiment ]
- 一般的method會 actively release memory during the backward pass, 所以almost constant wrt batch size in GB scale
-

** Over-parametrized $f_t$ **
As pointed out by R2, ``highly over-parametrized'' implies the parameter of each layer is in high dimension space. The description is usually used in deep learning literature [1-2] to indicate an optimization scheme where the dimension of the parameter is much higher than the data size. We revise the sentence in the revision to avoid the confusion.

[1] Empirical Analysis of the Hessian of Over-Parametrized Neural Networks
[2] How SGD Selects the Global Minima in Over-parameterized Learning: A Dynamical Stability Perspective


** Dimension of $Q^t_{uu}$ & matrix-free solver **
The dimension of $Q^t_{uu}$ is indeed quadratic in the number of parameter, $u \in \mathbb{R}^m$, of a single layer $t$. For fully-connected networks with the dimension of the hidden state being in $\mathbb{R}^n$,

We thank R2 for the



** Behavior of DDPNOpt2nd using ReLU **




We thank R2 for providing these detailed comments. We address all raised comments in the revision changes are marked with blue). Below we provide additional clarifications.

** Notation **
As pointed out by R2, we use $\mathcal{F}_t$ to denote any real-valued time-dependent function whereas
$\nabla_{\vx_t} \mathcal{F}_t$ denotes the first-order derivative of $\mathcal{F}_t$ evaluated on a given point $\vx_t$.
The abbreviations $\nabla_{\vx_t} \mathcal{F}_t \equiv \mathcal{F}^t_{\vx}$ is made so as to align with the notational convention in the DDP literature [1-3].

Unfortunately, we are not able Due to space constraint

Instead, we attach the corresponding equation


The faded arrows are meant to indicate the forward differential process (by the legend)

line 7-9 in Alg 2.

Since the purpose of Fig 1 is to provide visualization aid when comparing Alg 1 and 2,
we can consider dropping the whole weight update phase if Alg 1 and 2 are sufficiently informative to highlight the difference.




** Fig 1 **
Fig 1 now appears when we discuss the connection between DDP and Back-propagation, so that the notations are properly introduced.

The red arrow in weight update phase indicates the computation $u \leftarrow u + \delta u^*$, where the 'update' is computed from either Backprop ($\delta u^*$) or DDP ($\delta u^*(\delta x) = k_t + K_t(\delta x)$ )


We correct Fig 1 in the revision.


** Others **
In the revised version, we correct all mentioned typos (order 'of magnitude') and include the definition of vector-tensor product (footnote 1 in page 3).



[1] Synthesis and Stabilization of Complex Behaviors through Online Trajectory Optimization
[2]
[3]

====================== R3 =======================

We thank R3 for the valuable suggestions. We have re-organized the presentation with several amendments in the revised version (changes are marked with blue). We summarize the changes below.

** Approximation and $V_{xx}$ regularization **
To highlight the role of approximation and $V_{xx}$ regularization, in Sec 1 we enumerate the key approximations and factorizations that enable the efficient usage of DDPNOpt. This includes (i) curvature estimation from existing methods, (ii) stabilization techniques used in trajectory optimization, and (iii) efficient factorization to OCP. Discussion and derivation on each component are now grouped in Sec 3.2 (titled 'Efficient Approximation and Factorization') to highlight its importance. We also add additional discussion regarding the effect of $V_{xx}$ regularization on both traditional trajectory optimization and DNN training in page 6.


** Implementation of the final algorithm **
The pseudo-code of DDPNOpt is now attached in page 6 (Algorithm 3) right after we introduce DDPNOpt (Sec 3.2). The pseudo-code links the computation at each stage to the corresponding equation in the derivation section. For instance, derivatives of $Q_t$ with layer dynamics (Eq 12) is updated with only first-order expansion on the dynamics, which are used in the final algorithm. We hope the change will make it clear which equations are used in the final implementation.
The 'implementation detail' is now replaced with a full paragraph discussing the effect of $V_{xx}$ regularization.


Below we provide additional clarifications.

** Second-order method **
Despite dropping the second-order expansion on the dynamics, DDPNOpt still performs second-order expansions on the value function and propagates these Hessians (i.e. $V_{xx}$) backward through the layers, together with the first-order derivatives (Fig 1). We note that this optimization scheme, i.e. computing layer-wise Hessian with only linearized layer dynamics is closely related to the Gauss-Newton method [1], which can be related to the Natural Gradient method such as KFAC (see for instance Appendix C in [1]). Since both have been recognized as second order optimizers, we adopt the convention and identify DDPNOpt as second-order method.

As for the standard convergence analysis, DDP exhibits similar locally quadratic convergence as Newton when the dynamics is fully expanded to second order. We clarify this aspect in the revision when comparing DDP to Newton (page 7, 'Remarks on other optimizers.')

[1] Practical Gauss-Newton Optimisation for Deep Learning




While both (\eq{\ref{eq:Qt}} and \ref{eq:q-fc}) are considered second-order methods since second-order derivatives, \eg $\Vhht$ and $\Quxt$, are preserved in order to generate feedback policies, the latter can be thought of as performing Gauss-Newton approximation.}


====================== R4 =======================


** Organization **
We thank R4 for the valuable suggestion. In the revised version, we introduce DDPNOpt right after we present DDP and its connection to existing methods, so that the derivation of DDPNOpt is close to DDP. We hope this revision makes it easier to compare between these three frameworks. Discussion on 'Role of the feedback $K_t$ and $\delta x_t$ (i.e. the latter part of Sec 3 in the original submission) now appears after the derivation of DDPNOpt. As mentioned by R1 and R2, presentation of the connection between DDP and BP in the early text provides useful referencing point (and motivation) for the later derivation. We hope this organization improves the reading experience for a broader audience.


** Network architecture **
The feedforward networks (upper half of Table 3) consist of 5 fully-connected layers with the hidden dimension ranging from 10 to 32, depending on the size of dataset. Convolution networks (bottom half of Table 3) consist of 4 convolution layers (with 3 × 3 kernels), followed by 2 fully-connected layers. All networks use ReLU activation, except Tanh for WINE and DIGITS, with affine mapping at the final prediction layer.

Runtime comparison (Fig 3) reports the values with the same CNN model, but the relative performance between different optimizers remains similar for feedforward networks. Discussion on the feedback policies (Fig 4 and 6) is measured on DIGITS dataset; hence conducted with feedforward networks. Finally, Fig 5 visualizes the feedback policies when training CNNs. We include all clarifications (network architecture for each experiment) in the revised version (marked with blue in Sec 5).

In this paper we focus mainly on evaluating the performance of DDPNOpt with networks consisting of fully-connected and convolution layers. We note that when connecting modern architectures, e.g. (overlapping) residual connections, to the presenting optimal control perspective, the dynamical system interpretation of DNN (Eq 6) will require additional modifications. Since the dynamics is no longer a Markovian process, solving the Bellman equation (Eq 1) involves variables from earlier stages. We believe this will be an interesting direction to pursue in future works.


** SGD with momentum **
We thank R4 for pointing this out. Table 3 in the revised version now reports the training performance of SGD tuned with momentum. We find an improvement in accuracy when training with CNNs. We also note that DDPNOpt sustains the same position when comparing with existing methods.


** Performance on varying batch size **

Our experiment
We include all clarifications (network architecture for each experiment) in the revised version (marked with blue in Sec 5).


=================================================

DDPNOpt

Experiments
- setup for numerical complexity
- VG的實驗一定要加一些在main text, either text or fig


Appendix
- detailed complexity table (don't drop terms)



